Data-to-text Generation with Variational Sequential Planning

We consider the task of data-to-text generation, which aims to create textual output from non-linguistic input. We focus on generating long-form text, i.e., documents with multiple paragraphs, and propose a neural model enhanced with a planning component responsible for organizing high-level information in a coherent and meaningful way. We infer latent plans sequentially with a structured variational model, while interleaving the steps of planning and generation. Text is generated by conditioning on previous variational decisions and previously generated text. Experiments on two data-to-text benchmarks (RotoWire and MLB) show that our model outperforms strong baselines and is sample efficient in the face of limited training data (e.g., a few hundred instances).

==> sec_conclusion.tex <==
In this work, we proposed a novel sequential latent variable model for
joint macro planning and generation. Key in our approach is the
creation of a latent plan in a sequential manner, while interleaving
the prediction of plans and the generation of corresponding
paragraphs.  We propose to deconstruct monolithic long document
generation into  smaller units (paragraphs in our
case) which affords flexibility and better communication between
planning and generation. We experimentally show that our model
improves the factuality of long documents and is sample efficient when
evaluated on low resource settings.


